Gaia DR2 in 6D: Searching for the fastest stars in the Galaxy

We search for the fastest stars in the subset of stars with radial velocity measurements of the second data release (DR2) of the European Space Agency mission Gaia. Starting from the observed positions, parallaxes, proper motions, and radial velocities, we construct the distance and total velocity distribution of more than $7$ million stars in our Milky Way, deriving the full 6D phase space information in Galactocentric coordinates. These information are shared in a catalogue, publicly available at http://home.strw.leidenuniv.nl/~marchetti/research.html. To search for unbound stars, we then focus on stars with a probability greater than $50 \%$ of being unbound from the Milky Way. This cut results in a clean sample of $125$ sources with reliable astrometric parameters and radial velocities. Of these, $20$ stars have probabilities greater than 80 $\%$ of being unbound from the Galaxy. On this latter sub-sample, we perform orbit integration to characterize the stars' orbital parameter distributions. As expected given the relatively small sample size of bright stars, we find no hypervelocity star candidates, stars that are moving on orbits consistent with coming from the Galactic Centre. Instead, we find $7$ hyper-runaway star candidates, coming from the Galactic disk. Surprisingly, the remaining $13$ unbound stars cannot be traced back to the Galaxy, including two of the fastest stars (around $700$ km/s). If conformed, these may constitute the tip of the iceberg of a large extragalactic population or the extreme velocity tail of stellar streams.

==> tab_candidates_old.tex <==
\begin{landscape}
\begin{table}
\centering
\caption{Observed and derived properties for the $28$ "clean" high velocity star candidates with a probability $> 50\%$ of being unbound from the Galaxy.}
\label{tab:candidates}

\begin{threeparttable}

\begin{tabular}{lccccccccccc}

\hline
\Gaia DR2 ID & (RA, Dec.) & $\varpi$ & $\mu_{\alpha*}$ & $\mu_\delta$ & $v_\mathrm{rad}$ & $G$ & $d$ & $r_\mathrm{GC}$ & $v_\mathrm{GC}$ & $P_\mathrm{MW}$ & $P_\mathrm{ub}$ \\
 & ($^\circ$) & (mas) & (mas yr$^{-1}$) & (mas yr$^{-1}$) & (km s$^{-1}$) & (mag) & (pc) & (pc) & (\kms) &  &  \\
\hline


\textbf{HVS candidates} \\[0.15cm]

6397497209236655872 & ($333.11342$, $-68.1686$) & $0.173 \pm 0.017$ & $-18.709 \pm 0.022$ & $-6.567 \pm 0.026$ & $-8.158 \pm 3.613$ & $13.21$ & $5805^{+578}_{-491}$ & $6777^{+115}_{-60}$ & $587^{+49}_{-42}$& $0.24$ & $0.85$  \\[0.15cm] 
1364548016594914560 & ($268.77922$, $50.57305$) & $0.096 \pm 0.019$ & $-4.386 \pm 0.035$ & $7.819 \pm 0.038$ & $110.361 \pm 0.436$ & $11.93$ & $10309^{+2321}_{-1682}$ & $11951^{+1802}_{-1182}$ & $531^{+77}_{-53}$& $1.00$ & $0.74$  \\[0.15cm] 
6639557580310606976 & ($287.9278$, $-57.80599$) & $0.081 \pm 0.033$ & $-7.267 \pm 0.058$ & $2.431 \pm 0.05$ & $-257.081 \pm 1.196$ & $12.26$ & $11288^{+3426}_{-2327}$ & $6209^{+2749}_{-1349}$ & $581^{+94}_{-57}$ & $0.38$ & $0.62$  \\[0.15cm] 
4593398670455374592 & ($274.89655$, $33.81894$) & $0.201 \pm 0.022$ & $-1.185 \pm 0.036$ & $-25.738 \pm 0.041$ & $-312.966 \pm 1.157$ & $12.24$ & $4982^{+587}_{-483}$ & $7437^{+124}_{-69}$ & $545^{+71}_{-57}$& $0.55$ & $0.58$ \\[0.15cm]
1508756353921427328 & ($210.20492$, $45.86615$) & $0.148 \pm 0.024$ & $-15.547 \pm 0.033$ & $4.975 \pm 0.035$ & $128.221 \pm 1.289$ & $12.63$ & $6795^{+1214}_{-889}$ & $10693^{+817}_{-548}$ & $515^{+78}_{-53}$  & $0.99$& $0.58$ \\[0.15cm] 



\textbf{HRS candidates} \\[0.15cm]


5932173855446728064 & ($244.1181$, $-54.44045$) & $0.454 \pm 0.029$ & $-2.676 \pm 0.043$ & $-4.991 \pm 0.034$ & $-614.286 \pm 2.492$ & $13.81$ & $2205^{+126}_{-134}$ & $6391^{+103}_{-96}$ & $747^{+2}_{-3}$ & $0.02$& $1.00$  \\[0.15cm] 
5935868592404029184 & ($253.90291$, $-53.29868$) & $0.074 \pm 0.021$ & $5.47 \pm 0.032$ & $6.358 \pm 0.026$ & $308.412 \pm 1.212$ & $13.08$ & $12373^{+3060}_{-2480}$ & $6165^{+2667}_{-1768}$ & $755^{+118}_{-94}$& $0.45$ & $0.98$  \\[0.15cm] 
5244448023850619648 & ($153.90438$, $-69.19268$) & $0.054 \pm 0.013$ & $5.429 \pm 0.024$ & $-1.216 \pm 0.022$ & $39.876 \pm 3.525$ & $13.21$ & $16038^{+3405}_{-1976}$ & $15388^{+3024}_{-1672}$ & $540^{+84}_{-49}$& $0.18$ & $0.90$ \\[0.15cm] 
6431596947468407552 & ($274.68792$, $-70.24932$) & $0.084 \pm 0.016$ & $4.551 \pm 0.019$ & $4.974 \pm 0.023$ & $259.079 \pm 1.653$ & $13.09$ & $11910^{+2778}_{-1779}$ & $7936^{+2203}_{-1184}$ & $607^{+86}_{-56}$& $0.74$ & $0.87$  \\[0.15cm] 
5212817273334550016 & ($107.19916$, $-76.21933$) & $0.262 \pm 0.021$ & $12.169 \pm 0.039$ & $35.917 \pm 0.045$ & $159.866 \pm 0.278$ & $10.89$ & $3826^{+294}_{-288}$ & $8039^{+63}_{-51}$ & $568^{+52}_{-51}$& $0.35$ & $0.79$  \\[0.15cm]
3705761936916676864 & ($192.7642$, $4.94109$) & $0.266 \pm 0.024$ & $15.037 \pm 0.053$ & $-32.292 \pm 0.032$ & $88.655 \pm 1.877$ & $13.19$ & $3736^{+397}_{-303}$ & $8289^{+108}_{-70}$ & $564^{+63}_{-47}$ & $0.30$& $0.79$  \\[0.15cm] 
6077622510498751616 & ($187.9836$, $-53.91915$) & $0.054 \pm 0.02$ & $-6.685 \pm 0.022$ & $1.212 \pm 0.022$ & $623.609 \pm 0.81$ & $13.06$ & $15014^{+3626}_{-3152}$ & $13073^{+3161}_{-2502}$ & $548^{+81}_{-59}$ & $0.99$& $0.79$  \\[0.15cm] 
2233912206910720000 & ($299.2838$, $55.49696$) & $0.278 \pm 0.018$ & $27.848 \pm 0.031$ & $-5.483 \pm 0.034$ & $-343.939 \pm 1.714$ & $12.97$ & $3595^{+227}_{-236}$ & $8895^{+91}_{-89}$ & $540^{+30}_{-31}$ & $0.42$& $0.76$  \\[0.15cm] 
4531575708618805376 & ($281.8599$, $22.13939$) & $0.08 \pm 0.018$ & $4.073 \pm 0.017$ & $5.153 \pm 0.031$ & $-417.36 \pm 0.895$ & $13.06$ & $11898^{+2687}_{-2049}$ & $9587^{+2104}_{-1372}$ & $558^{+79}_{-58}$& $0.34$  & $0.73$ \\[0.15cm] 
5374177064347894272 & ($169.49883$, $-47.83129$) & $0.168 \pm 0.025$ & $7.244 \pm 0.041$ & $-17.28 \pm 0.037$ & $143.173 \pm 0.453$ & $12.19$ & $5975^{+1013}_{-837}$ & $8644^{+470}_{-315}$ & $566^{+87}_{-72}$ & $0.35$& $0.72$  \\[0.15cm]
6010197124582216832 & ($239.83557$, $-37.75698$) & $0.084 \pm 0.027$ & $8.038 \pm 0.054$ & $-1.178 \pm 0.034$ & $294.687 \pm 2.935$ & $13.95$ & $11267^{+3017}_{-2103}$ & $5009^{+2534}_{-1310}$ & $643^{+105}_{-71}$& $0.28$ & $0.71$ \\[0.15cm] 
5779439836114210304 & ($234.18614$, $-78.30489$) & $0.014 \pm 0.015$ & $1.207 \pm 0.022$ & $2.469 \pm 0.025$ & $12.004 \pm 1.049$ & $13.36$ & $23333^{+6165}_{-4603}$ & $19311^{+5899}_{-4265}$ & $485^{+74}_{-55}$& $0.33$ & $0.69$ \\[0.15cm]
4916199478888664320 & ($23.38253$, $-51.92318$) & $0.184 \pm 0.023$ & $-11.091 \pm 0.034$ & $-17.585 \pm 0.036$ & $86.865 \pm 1.326$ & $12.61$ & $5457^{+691}_{-599}$ & $9211^{+345}_{-267}$ & $538^{+62}_{-53}$& $0.44$ & $0.67$  \\[0.15cm] 
3784964943489710592 & ($169.3563$, $-5.81538$) & $0.259 \pm 0.039$ & $22.575 \pm 0.077$ & $-16.335 \pm 0.048$ & $126.155 \pm 1.27$ & $12.25$ & $3883^{+711}_{-494}$ & $9273^{+354}_{-222}$ & $534^{+87}_{-59}$ & $0.49$& $0.63$  \\[0.15cm] 
1268023196461923712 & ($225.78358$, $26.24632$) & $0.224 \pm 0.022$ & $-29.641 \pm 0.039$ & $-18.877 \pm 0.041$ & $-276.839 \pm 1.644$ & $13.00$ & $4482^{+507}_{-410}$ & $7698^{+105}_{-61}$ & $551^{+80}_{-63}$ & $0.49$& $0.62$ \\[0.15cm] 
1042515801147259008 & ($129.79902$, $62.50127$) & $0.389 \pm 0.034$ & $-33.08 \pm 0.035$ & $-41.029 \pm 0.067$ & $73.916 \pm 1.144$ & $12.72$ & $2588^{+217}_{-219}$ & $10228^{+182}_{-182}$ & $518^{+50}_{-49}$& $0.56$ & $0.60$  \\[0.15cm]
5847044923481848192 & ($210.57$, $-69.36009$) & $0.062 \pm 0.015$ & $3.313 \pm 0.022$ & $3.851 \pm 0.023$ & $74.408 \pm 1.095$ & $13.53$ & $14846^{+3075}_{-2370}$ & $11628^{+2668}_{-1892}$ & $513^{+71}_{-55}$ & $0.49$& $0.60$ \\[0.15cm] 
4248140165233284352 & ($299.668$, $4.51105$) & $0.147 \pm 0.021$ & $-17.336 \pm 0.034$ & $-0.186 \pm 0.026$ & $-358.1 \pm 2.283$ & $13.21$ & $6725^{+1179}_{-772}$ & $6017^{+314}_{-83}$ & $567^{+89}_{-56}$ & $0.50$& $0.56$ \\[0.15cm] 
5823263311601403392 & ($231.31938$, $-68.50629$) & $0.111 \pm 0.026$ & $7.405 \pm 0.027$ & $-4.895 \pm 0.041$ & $-78.245 \pm 0.699$ & $12.64$ & $9078^{+2148}_{-1580}$ & $6600^{+1279}_{-614}$ & $557^{+78}_{-56}$ & $1.00$& $0.55$ \\[0.15cm] 
5508788005188732416 & ($107.05511$, $-48.32651$) & $0.216 \pm 0.022$ & $22.734 \pm 0.043$ & $-13.23 \pm 0.039$ & $257.033 \pm 2.069$ & $12.55$ & $4623^{+533}_{-442}$ & $10124^{+331}_{-261}$ & $510^{+66}_{-55}$ & $0.62$& $0.54$  \\[0.15cm] 
4536536670713820288 & ($276.23382$, $24.0701$) & $0.1 \pm 0.015$ & $-8.548 \pm 0.017$ & $-8.547 \pm 0.026$ & $-501.403 \pm 2.331$ & $13.60$ & $10177^{+1649}_{-1364}$ & $8505^{+1121}_{-783}$ & $527^{+80}_{-62}$ & $0.60$& $0.53$ \\[0.15cm]
2036303544778830080 & ($288.22674$, $26.8623$) & $0.131 \pm 0.02$ & $12.347 \pm 0.027$ & $-0.824 \pm 0.035$ & $-100.043 \pm 1.191$ & $13.02$ & $7632^{+1459}_{-1081}$ & $7883^{+744}_{-414}$ & $536^{+83}_{-61}$ & $0.54$ & $0.54$ \\[0.15cm] 
5482348392671802624 & ($91.55732$, $-60.34047$) & $0.133 \pm 0.012$ & $3.182 \pm 0.021$ & $13.026 \pm 0.023$ & $434.118 \pm 2.079$ & $13.16$ & $7609^{+790}_{-583}$ & $11247^{+555}_{-391}$ & $497^{+44}_{-33}$ & $0.99$& $0.52$  \\[0.15cm] 




\hline
\end{tabular}

\begin{tablenotes}

\item \emph{Note.} Distances and total velocities are quoted in terms of the median of the distribution, with uncertainties derived from the $16$th and $84$th percentiles.

\end{tablenotes}

\end{threeparttable}
\end{table}
\end{landscape}
